Streaming PTAS for Binary $\ell_0$-Low Rank Approximation

We give a 3-pass, polylog-space streaming PTAS for the constrained binary $k$-means problem and a 4-pass, polylog-space streaming PTAS for the binary $\ell_0$-low rank approximation problem. The connection between the above two problems has recently been studied. We design a streaming PTAS for the former and use this connection to obtain streaming PTAS for the latter. This is the first constant pass, polylog-space streaming algorithm for either of the two problems.

==> binary-k-means.tex <==
Recall that the binary $k$-means problem is defined in the following manner: Given $n$ points $X \subseteq \{0, 1\}^d$ and an integer $k$, find a set $C \subseteq \{0, 1\}^d$ of $k$ centers such that the following cost function is minimised: 
\[
\Phi(C, X) \equiv \sum_{x \in X} \min_{c \in C} \norm{x - c}^2
\]
The binary 1-means problem is computationally easy (as is the standard 1-means problem). 
The optimal center for the 1-means problem simply has the majority bit in each of the $d$ coordinates. 
However, the problem becomes $\mathsf{NP}$-hard for $k > 1$ \cite{kpr98}.
Due to the similarity of the binary-$k$-means problem to the standard $k$-means problem, where the point set $X$ and centers $C$ are allowed to be from $\R^d$ instead of $\{0, 1\}^d$, let us quickly check whether an approximation algorithm for the standard $k$-means problem also gives an approximation algorithm for the binary $k$-means problem. This indeed is true and the following simple lemma summarises this.

\begin{lemma}\label{lemma:simple-fact}
Let $\tt{Alg}$ be an $\alpha$-approximation algorithm for the standard $k$-means problem, then the following algorithm $\tt{Algb}$ is a $4 \alpha$-approximation algorithm for the binary $k$-means problem.
\begin{framed}
{\tt Algb($X, k$)} \\
\hspace*{0.3in} -  Let $C \leftarrow$ {\tt Alg($X, k$)} and let $C' \leftarrow \emptyset$\\
\hspace*{0.3in} - For every $c \in C$:\\
\hspace*{0.6in} - Let $c' \leftarrow \arg\min_{x \in X} \norm{x - c}^2$ and let $C' \leftarrow C' \cup \{c'\}$\\
\hspace*{0.3in} - return($C'$)
\end{framed}
\end{lemma}
\begin{proof}
Let $OPT$ denote the optimal standard $k$-means cost for the input instance $(X, k)$ and let $OPTB$ denote the optimal binary $k$-means cost. Clearly, $OPT \leq OPTB$.
Since $C$ is an $\alpha$-approximate solution,  we have $\Phi(C, X) \leq \alpha \cdot OPT$. For any center $c \in C$ and set of points $S \subseteq X$, let $N(c, S) \equiv \arg\min_{s \in S} \norm{s - c}^2$. 
Let $X_1', X_2', ..., X_k'$ be the clustering of $X$ induced by the center set $C' = \{c_1', ..., c_k'\}$ and $X_1, ..., X_k$ be the clusters induced by the corresponding centers in $C = \{c_1, ..., c_k\}$.
Then we have:
\begin{eqnarray*}
\Phi(C', X) &=& \sum_{i=1}^{k} \sum_{x \in X_i'} \norm{x - c_i'}^2 \\
%
&\leq& \sum_{i=1}^{k} \sum_{x \in X_i} \norm{x - c_i'}^2 \qquad \textrm{(since $X_1', ..., X_k'$ is optimal w.r.t. $C'$)}\\
%
&\leq& 2 \cdot \sum_{i=1}^{k} \left( \sum_{x \in X_i} \norm{x - c_i}^2 + |X_i| \cdot \norm{c_i - c_i'}^2\right) \qquad \textrm{(using $\norm{p-r}^2 \leq 2 \norm{p-q}^2 + 2\norm{q-r}^2$)}\\
%
&=& 2 \cdot \sum_{i=1}^{k} \left( \sum_{x \in X_i} \norm{x - c_i}^2 + |X_i| \cdot \norm{c_i - N(c_i, X)}^2\right)\\
%
&\leq& 2 \cdot \sum_{i=1}^{k} \left( \sum_{x \in X_i} \norm{x - c_i}^2 + |X_i| \cdot \norm{c_i - N(c_i, X_i)}^2\right)\\
%
&\leq& 4 \cdot \sum_{i=1}^{k} \left( \sum_{x \in X_i} \norm{x - c_i}^2 \right) = (4 \alpha) \cdot OPT \leq (4 \alpha) \cdot OPTB
\end{eqnarray*}
This completes the proof of the lemma.\qed
\end{proof}


The above lemma tells us that if there is a single-pass streaming approximation algorithm for the standard $k$-means problem, then there is a 2-pass streaming approximation algorithm for the binary $k$-means problem.
Fortunately, there indeed exists such a single pass streaming approximation algorithm that gives constant approximation. One such algorithm was given by Charikar \etal~\cite{cop03} which was later improved by Braverman \etal~\cite{brav11}. We state the result of Braverman \etal~\cite{brav11} below for reference.

\begin{theorem}[Theorem 3.2 in \cite{brav11}]
There is a constant factor streaming algorithm for the standard $k$-means problem that runs in a single pass over the data while storing $O(k \log{n})$ points in memory with overall running time $O(nk \log{n})$.
\end{theorem}
Combining the above result of Braverman \etal with Lemma~\ref{lemma:simple-fact}, we get that the following result that will be used in the next section where we use this to obtain a solution for the constrained binary $k$-means problem.

\begin{theorem}
There is a constant factor streaming algorithm for the binary $k$-means problem that runs in two passes over the data while storing $O(k \log{n})$ point in memory with overall running time $O(nk \log{n})$.
\end{theorem}
The theorem follows from the simple observation that the streaming algorithm for the binary $k$-means problem runs the streaming algorithm of Braverman \etal in the first pass to obtain an approximate solution $C$ and in the second pass runs lines 2--4 of algorithm {\tt Algb} of Lemma~\ref{lemma:simple-fact}.
It should be noted that Lemma~\ref{lemma:simple-fact} is a known fact (though may not be known in the form given here) that has been used in the previous works on $k$-means clustering. 
We give this lemma explicitly for better readability.
